Common origin of quasi-periodic pulsations in microwave and decimetric solar radio bursts

We analyse quasi-periodic pulsations (QPP) detected in the microwave and decimeter radio emission of the SOL2017-09-05T07:04 solar flare, using simultaneous observations by the Siberian Radioheliograph 48 (SRH-48, 4-8 GHz) and Mingantu Spectral Radioheliograph (MUSER-I, 0.4-2 GHz). The microwave emission was broadband with a typical gyrosynchrotron spectrum, while a quasi-periodic enhancement of the decimetric emission appeared in a narrow spectral band (500-700 MHz), consistent with the coherent plasma emission mechanism. The periodicity that we found in microwaves is about 30 s, coming from a compact loop-like source with a typical height of about 31 Mm. The decimetric emission demonstrated a periodicity about 6 s. We suggested a qualitative scenario linking the QPPs observed in both incoherent and coherent spectral bands and their generation mechanisms. The properties of the QPPs found in the microwave signal are typical for perturbations of the flare loop by the standing sausage mode of a fast magnetohydrodynamic (MHD) wave. Our analysis indicated that this sausage-oscillating flare loop was the primary source of oscillations in the discussed event. The suggested scenario is that a fundamental sausage harmonic is the dominant cause for the observed QPPs in the microwave emission. The initiation of oscillations in the decimetric emission is caused by the third sausage harmonic via periodic and nonlinear triggering of the acceleration processes in the current sheets, formed at the interface between the sausage-oscillating flare loop and the external coronal loop that extended to higher altitudes. Our results demonstrate the possible role of MHD wave processes in the release and transport of energy during solar flares, linking coherent and incoherent radio emission mechanisms.

==> SOLA_example_labels.tex <==
This file contains the command names and the labels used in
the associated .tex file.    It is useful to have present file open
as the same time of the .tex file to copy/paste definitions.
When a new definition is added, it is important to keep this file
updated. 

   % Copy/paste of the definitions used in the .tex
\newcommand{\BibTeX}{\textsc{Bib}\TeX}
\newcommand{\etal}{{\it et al.}}

% Definitions for equations
\newcommand{\deriv}[2]{\frac{{\mathrm d} #1}{{\mathrm d} #2}}
\newcommand{\rmd}{ {\ \mathrm d} }
\renewcommand{\vec}[1]{ {\mathbf #1} }
\newcommand{\uvec}[1]{ \hat{\mathbf #1} }
\newcommand{\pder}[2]{ \f{\partial #1}{\partial #2} }
\newcommand{\grad}{ {\bf \nabla } }
\newcommand{\curl}{ {\bf \nabla} \times}
\newcommand{\vol}{ {\mathcal V} }
\newcommand{\bndry}{ {\mathcal S} }
\newcommand{\dv}{~{\mathrm d}^3 x}
\newcommand{\da}{~{\mathrm d}^2 x}
\newcommand{\dl}{~{\mathrm d} l}
\newcommand{\dt}{~{\mathrm d}t}
\newcommand{\intv}{\int_{\vol}^{}}
\newcommand{\inta}{\int_{\bndry}^{}}
\newcommand{\avec}{ \vec A}
\newcommand{\ap}{ \vec A_p}
\newcommand{\bb}{ \vec B}
\newcommand{\jj}{ \vec j}
\newcommand{\rr}{ \vec r}
\newcommand{\xx}{ \vec x}

% Definitions for the journal names
\newcommand{\adv}{    {\it Adv. Space Res.}} 
\newcommand{\annG}{   {\it Ann. Geophys.}} 
\newcommand{\aap}{    {\it Astron. Astrophys.}}
\newcommand{\aaps}{   {\it Astron. Astrophys. Suppl.}}
\newcommand{\aapr}{   {\it Astron. Astrophys. Rev.}}
\newcommand{\ag}{     {\it Ann. Geophys.}}
\newcommand{\aj}{     {\it Astron. J.}} 
\newcommand{\apj}{    {\it Astrophys. J.}}
\newcommand{\apjl}{   {\it Astrophys. J. Lett.}}
\newcommand{\apss}{   {\it Astrophys. Space Sci.}} 
\newcommand{\cjaa}{   {\it Chin. J. Astron. Astrophys.}} 
\newcommand{\gafd}{   {\it Geophys. Astrophys. Fluid Dyn.}}
\newcommand{\grl}{    {\it Geophys. Res. Lett.}}
\newcommand{\ijga}{   {\it Int. J. Geomagn. Aeron.}}
\newcommand{\jastp}{  {\it J. Atmos. Solar-Terr. Phys.}} 
\newcommand{\jgr}{    {\it J. Geophys. Res.}}
\newcommand{\mnras}{  {\it Mon. Not. Roy. Astron. Soc.}}
\newcommand{\nat}{    {\it Nature}}
\newcommand{\pasp}{   {\it Pub. Astron. Soc. Pac.}}
\newcommand{\pasj}{   {\it Pub. Astron. Soc. Japan}}
\newcommand{\pre}{    {\it Phys. Rev. E}}
\newcommand{\solphys}{{\it Solar Phys.}}
\newcommand{\sovast}{ {\it Soviet  Astron.}} 
\newcommand{\ssr}{    {\it Space Sci. Rev.}} 

%%%%%%%%%%%%%%%% Roadmap of the paper with all the labels %%%%%%%%%%%%%%%%%%%%%%%%
%%%% (with the exception of citations since author-year is easy to remember) %%%%%
1 Section~\ref{S-Introduction}
2 Section~\ref{S-general}
  Section~\ref{S-text}
  Section~\ref{S-labels}
3 Section~\ref{S-features}
  Section~\ref{S-equations}
   Section~\ref{S-simple-equations}
     Equation~(\ref{Eq-H-def})
   Section~\ref{S-array-equations}
     Equation~(\ref{Eq-A-B})
     Equation~(\ref{Eq-H-B})
     Equation~(\ref{Eq-H-N})
   Section~\ref{S-long-equations}
     Equation~(\ref{Eq-dH-Phi})  
  Section~\ref{S-figures}
  Section~\ref{S-tables}
  Section~\ref{S-references}
  Section~\ref{S-BibTeX}
  Section~\ref{S-Miscellaneous}
4 Section~\ref{S-Conclusion}

A Appendix~\ref{S-appendix}
 
 1 Figure~\ref{F-simple}
 2 Figure~\ref{F-4panels}
 3 Figure~\ref{F-rotate-cut}
 4 Figure~\ref{F-appendix}

 1 Table~\ref{T-simple}
 2 Table~\ref{T-complex}
 3 Table~\ref{T-appendix}

%%%%%%%%%%%%%%%%%%%% Results for the citation commands %%%%%%%%%%%%%%%%%%%%%%%%  
\cite{Kusano04}          : (Kusano \etal, 2004)
\cite{Kusano04,Berger03} : (Kusano \etal, 2004; Berger, 2003)
\inlinecite{Brown99}     : Brown, Canfield, and Pevtsov (1999)
\opencite{Brown99}       : Brown, Canfield, and Pevtsov, 1999
\citeauthor{Brown99}     : Brown, Canfield, and Pevtsov
\shortcite{Brown99}      : (1999)
\citeyear{Brown99}       : 1999
(\opencite{Berger84}, \citeyear{Berger03}) 
                         : (\opencite{Berger84}, \citeyear{Berger03})


